Random Linear Network Codes for Secrecy over Wireless Broadcast Channels

We consider a set of $n$ messages and a group of $k$ clients. Each client is privileged for receiving an arbitrary subset of the messages over a broadcast erasure channel, which generalizes scenario of a previous work. We propose a method for secretly delivering each message to its privileged recipients in a way that each receiver can decode its own messages but not the others'. Our method is based on combining the messages using linear network coding and hiding the decoding coefficients from the unprivileged clients. We provide an information theoretic proof for the secrecy of the proposed method. In particular we show that an unprivileged client cannot obtain any meaningful information even if it holds the entire set of coded data packets transmitted over the channel. Moreover, in our method, the decoding complexity is desirably low at the receiver side.

==> Conclusion.tex <==
\section{Discussion and Conclusion}\label{sec:Conclusion}
In this paper we introduced a method for maintaining the secrecy
over a wireless broadcast channel where each receiver is allowed to
obtain a subset of messages but not the entire set. Here some
specifications and advantages of the proposed method and some
potentials for future work are discussed:
%\begin{enumerate}
%\item We used the linear network codes in a reverse direction, i.e.
%instead of generating linear combinations of the messages
%($\mathbf{P}=\mathbf{A}\mathbf{X}$) and broadcasting them over the
%channel, a system of linear equations
%($\mathbf{X}=\mathbf{A}\mathbf{P}$) is solved at the base station to
%generate packets $P$. Therefore, each message is related to the set
%of packets with a distinct set of decoding coefficients which
%enables us to generalize the proposed method to the scenario that
%each client is interested in an arbitrary subset of messages without
%violating the secrecy of other clients (As each client is provided
%with only the decoding coefficients necessary for decoding the
%messages that he is privileged for).
%\item Reversing the direction of coding scheme mentioned in the last
%item, also has the advantage that reduces the complexity at the
%receiver side which might potentially have limited power resource
%and computational capacity. In our proposed scheme, the receiver
%only needs to compute a linear combination of packets for each
%message instead of inverting a matrix.
%\item The role of regenerating vector is to update the decoding
%coefficients to maintain the uniformity of the decoding coefficients
%distribution. However, we conjecture that leakage of information
%(even about the joint distribution of messages) is negligible with
%updating the decoding coefficients even if the distribution of
%messages is not uniform. The role of permutation functions in the
%initial keys is to produce a huge space of possibilities that makes
%it computationally hard to guess the decoding coefficients or obtain
%any information about them. The amount of leakage of information in
%the case of non-uniform messages is an interesting topic for further
%investigation. However,the regenerating vector does not need to be
%updated necessarily  at each round and can be updated periodically
%after several rounds of transmission.  If the amount of information
%leakage for the case of non-uniform messages is characterized, the
%appropriate length of updating regenerating period can be
%identified.
%\end{enumerate}

